Tea: Program Repair Using Neural Network Based on Program Information Attention Matrix

The advance in machine learning (ML)-driven natural language process (NLP) points a promising direction for automatic bug fixing for software programs, as fixing a buggy program can be transformed to a translation task. While software programs contain much richer information than one-dimensional natural language documents, pioneering work on using ML-driven NLP techniques for automatic program repair only considered a limited set of such information. We hypothesize that more comprehensive information of software programs, if appropriately utilized, can improve the effectiveness of ML-driven NLP approaches in repairing software programs. As the first step towards proving this hypothesis, we propose a unified representation to capture the syntax, data flow, and control flow aspects of software programs, and devise a method to use such a representation to guide the transformer model from NLP in better understanding and fixing buggy programs. Our preliminary experiment confirms that the more comprehensive information of software programs used, the better ML-driven NLP techniques can perform in fixing bugs in these programs.

==> tex/F_conclusion.tex <==
\section{Conclusion}
Based on the neural network transformer model, we proposed to use program analysis to construct the program representation attention matrix PIAM, and finally realized the error repair model Tea. Compared with the previous method, we consider the difference between programming language and natural language, and use the method of program analysis to construct an attention matrix based on program representation, so that the neural network can smoothly learn more program information, thereby improving the program repair accuracy.


==> tex/G_Ack.tex <==
\section*{Acknowledgements}
% \section{Acknowledgments}
We sincerely appreciate the anonymous reviewers for their insightful comments and feedback. This research is supported in part by National Natural Science Foundations of China (Grant No.61772506 and No.62072448) and National Key R\&D Program of China (Grant No. 2017YFB0802902).
